MIDIS: JWST/MIRI reveals the Stellar Structure of ALMA-selected Galaxies in the Hubble-UDF at Cosmic Noon

We present deep James Webb Space Telescope (JWST)/MIRI F560W observations of a flux-limited, ALMA-selected sample of 28 galaxies at z=0.5-3.6 in the Hubble Ultra Deep Field (HUDF). The data from the MIRI Deep Imaging Survey (MIDIS) reveal the stellar structure of the HUDF galaxies at rest-wavelengths of >1 micron for the first time. We revise the stellar mass estimates using new JWST photometry and find good agreement with pre-JWST analysis; the few discrepancies can be explained by blending issues in the earlier lower-resolution Spitzer data. At z~2.5, the resolved rest-frame near-infrared (1.6 micron) structure of the galaxies is significantly more smooth and centrally concentrated than seen by HST at rest-frame 450 nm (F160W), with effective radii of Re(F560W)=1-5 kpc and S\'ersic indices mostly close to an exponential (disk-like) profile (n~1), up to n~5 (excluding AGN). We find an average size ratio of Re(F560W)/Re(F160W)~0.7 that decreases with stellar mass. The stellar structure of the ALMA-selected galaxies is indistinguishable from a HUDF reference sample of galaxies with comparable MIRI flux density. We supplement our analysis with custom-made, position-dependent, empirical PSF models for the F560W observations. The results imply that a smoother stellar structure is in place in massive gas-rich, star-forming galaxies at Cosmic Noon, despite a more clumpy rest-frame optical appearance, placing additional constraints on galaxy formation simulations. As a next step, matched-resolution, resolved ALMA observations will be crucial to further link the mass- and light-weighted galaxy structures to the dusty interstellar medium.

==> affiliations.tex <==
\newcommand{\MPIA}{\affiliation{Max Planck Institute for Astronomy, K\"onigstuhl 17,  69117 Heidelberg, Germany}}

\newcommand{\DAWN}{\affiliation{Cosmic Dawn Center (DAWN), Denmark}}

\newcommand{\DTU}{\affiliation{DTU Space, Technical University of Denmark, Elektrovej, Building 328, 2800, Kgs. Lyngby, Denmark}}

\newcommand{\DARK}{\affil{DARK, Niels Bohr Institute, University of Copenhagen, Jagtvej 128, 2200 Copenhagen, Denmark}}

\newcommand{\Stockholm}{\affiliation{Department of Astronomy, Stockholm University, Oscar Klein Centre, AlbaNova University Centre, 106 91 Stockholm, Sweden}}

\newcommand{\NRAO}{\affiliation{National Radio Astronomy Observatory, Pete V. Domenici Array Science Center, P.O. Box O, Socorro, NM 87801, USA}}

\newcommand{\CABcda}{\affiliation{Centro de Astrobiolog\'{i}a (CAB), CSIC-INTA, Ctra. de Ajalvir km 4, Torrej\'{o}n de Ardoz, E-28850, Madrid, Spain}}
\newcommand{\CABcbdc}{\affiliation{Centro de Astrobiolog\'{i}a (CAB), CSIC-INTA, Camino Bajo del Castillo s/n, 28692 Villanueva de la Ca\~{n}ada, Madrid, Spain}}

\newcommand{\ESAC}{\affiliation{Telespazio UK for the European Space Agency, ESAC, Camino Bajo del Castillo s/n, 28692 Villanueva de la Ca\~nada, Spain}}

\newcommand{\Kapteyn}{\affiliation{Kapteyn Astronomical Institute, University of Groningen, P.O. Box 800, 9700AV Groningen, The Netherlands}}

\newcommand{\Leiden}{\affil{Leiden Observatory,  Leiden University, PO Box 9513, NL-2300 RA Leiden, The Netherlands}}

\newcommand{\UCL}{\affiliation{Dept. of Physics and Astronomy, University College London, Gower Street, London WC1E 6BT, United Kingdom}}

\newcommand{\Edinburgh}{\affiliation{UK Astronomy Technology Centre, Royal Observatory Edinburgh, Blackford Hill, Edinburgh EH9 3HJ, UK}}

\newcommand{\ITA}{\affil{Institute for Theoretical Physics, Heidelberg University, Philosophenweg 12, D–69120, Heidelberg, Germany}}

\newcommand{\Cologne}{\affil{I.Physikalisches Institut der Universit\"{a}t zu K\"{o}ln, Z\"{u}lpicher Str. 77, 50937 K\"{o}ln, Germany}}

\newcommand{\MPIfR}{\affil{Max Planck Institute for Radiosastronomie, Auf dem H\"{u}gel 69, 53121 Bonn, Germany}}

\newcommand{\Geneva}{\affil{Departement d'Astronomie, University of Geneva, Chemin Pegasi 51, 1290 Versoix, Switzerland}}

\newcommand{\Marseille}{\affil{Aix Marseille Univ, CNRS, CNES, LAM, Marseille, France}}

\newcommand{\SPL}{\affil{School of Physics \& Astronomy, Space Research Centre, Space Park Leicester, University of Leicester, 92 Corporation Road, Leicester LE4 5SP, UK}}

\newcommand{\Dublin}{\affil{Dublin Institute for Advanced Studies, Astronomy \& Astrophysics Section, 31 Fitzwilliam Place, Dublin 2, Ireland}}

